The probabilistic world

Physics is based on probabilities as fundamental entities of a mathematical description. Expectation values of observables are computed according to the classical statistical rule. The overall probability distribution for one world covers all times. The quantum formalism arises once one focuses on the evolution of the time-local probabilistic information. Wave functions or the density matrix allow the formulation of a general linear evolution law for classical statistics. The quantum formalism for classical statistics is a powerful tool which allows us to implement for generalized Ising models the momentum observable with the associated Fourier representation. The association of operators to observables permits the computation of expectation values in terms of the density matrix by the usual quantum rule. We show that probabilistic cellular automata are quantum systems in a formulation with discrete time steps and real wave functions. With a complex structure the evolution operator for automata can be expressed in terms of a Hamiltonian involving fermionic creation and annihilation operators. The time-local probabilistic information amounts to a subsystem of the overall probabilistic system which is correlated with its environment consisting of the past and future. Such subsystems typically involve probabilistic observables for which only a probability distribution for their possible measurement values is available. Incomplete statistics does not permit to compute classical correlation functions for arbitrary subsystem-observables. Bell's inequalities are not generally applicable.

==> 2_5_5__Normalized_classical_wave_function.tex <==
\subsubsection{Normalized classical wave function}

The normalized classical wave function [54]\todo{ref} is a powerful tool for the discussion of entanglement in classical probabilistic
systems. It provides for classical statistics a formulation in close analogy to quantum mechanics. This makes the similarity between
quantum entanglement and classical entanglement particularly apparent. 

\paragraph*{Classical wave function and probabilities}

We define the normalized classical wave function $q$ as a root of the probability distribution 
\begin{equation}
\label{eq:E59}
p_\tau = q_\tau^2\,.
\end{equation}
This determines $q_\tau$ up to a sign $\sigma_\tau$,
\begin{equation}
\label{eq:E60}
q_\tau = \sigma_\tau \sqrt{p_\tau}\,, \quad \sigma_\tau = \pm 1\,.
\end{equation}
The normalization of the probabilities $\sum_\tau p_\tau = 1$ implies that q is a uni vector,
\begin{equation}
\label{eq:E61}
q_\tau q_\tau = 1\,.
\end{equation}
Transformations of the probability distribution that preserve the normalization are simply rotations of the normalized wave function.
This implicitly is an important advantage for many purposes. 

We have encountered in the discussion of local chains in \ref{sec:2_2_3__}\todo{ref doesn't exist yet} a pair of classical wave functions
$\tilde{q}_\tau$ and conjugate wave function $\bar{q}_\tau$. They can be used to define the normalized classical wave function, using the 
relation (no sum over $\tau$)
\begin{equation}
\label{eq:E62}
q_\tau q_\tau = \bar{q}_\tau \tilde{q}_\tau = p_\tau\,.
\end{equation}
We may define [2] 
\begin{equation}
\label{eq:E63}
q_\tau = \sign(\tilde{q}_\tau) \sqrt{\bar{q}_\tau \tilde{q}_\tau}\,.
\end{equation}
The map from the pair of classical wave functions $(\tilde{q}_\tau,\bar{q}_\tau )$ to the normalized classical wave function $q_\tau$ 
is, in general, non-linear. For the special case of an orthogonal step evolution operator and suitable boundary conditions one has 
for all $t$ the relation $\bar{q}_\tau = \tilde{q}_\tau$. In this case one finds the simple relation
\begin{equation}
\label{eq:E64}
q_\tau = \tilde{q}_\tau = \bar{q}_\tau \,.
\end{equation}

Using the classical operators $\hat{A}$ introduced in sect. \ref{sec:2_2_3} one finds for the expectation value a relation similar to 
quantum mechanics. 
\begin{equation}
\label{eq:E65}
\braket{A} = q_\tau \hat{A}_{\tau \rho} q_\rho = \braket{q | \hat{A} | q}\,.
\end{equation}
With the identification \eqref{eq:E63} this coincides with eq.~(2.2.45)\todo{lookup ref} for diagonal classical operators 
\begin{equation}
\label{eq:E66}
\hat{A}_{\tau \rho} = A_\tau \delta_{\tau \rho}\,.
\end{equation}
The signs $\sigma_\tau$ drop out for diagonal classical operators. Eq.~\eqref{eq:E65} reproduces directly the fundamental definition 
of expectation values (2.1.2) in classical statistics
\begin{equation}
\label{eq:E67}
\sum_{\tau, \rho} q_\tau \hat{A} q_\rho = \sum_\tau A_\tau q_\tau^2 = \sum_\tau A_\tau p_\tau\,.
\end{equation}

\paragraph*{Classical entanglement}

In the formalism for normalized classical wave functions we can directly implement concepts familiar from quantum mechanics as direct
product wave functions and entanglement wave functions. As in quantum mechanics, the notions of direct product and entanglement depend
on the definition of parts of the system and the adapted choice of basis functions.

In the two-particle basis the six classical spin operators corresponding to the Ising spins $s_k^{(1)}, s_k^{(2)}$ are represented as
\begin{equation}
\label{eq:E68}
\hat{S}_k^{(1)} = \hat{S}_k \otimes 1\,, \quad \hat{S}_k^{(1)} =  1 \otimes \hat{S}_k\,,
\end{equation}
with diagonal $8 \times 8$ matrices $\hat{S}_k$ given by eqs. (2.4.6), (2.4.4). A direct product normalized wave function take the
form 
\begin{equation}
\label{eq:E69}
q_\tau = q_{\tau_1 \tau_2} = q_{\tau_1}^{(1)} q_{\tau_2}^{(2)}\,,
\end{equation}
with 8-component uni vectors $q^{(1)}$ and $q^{(2)}$. For direct product wave functions one has
\begin{equation}
\label{eq:E70}
p_\tau = p_{\tau_1}^{(1)} p_{\tau_2}^{(2)}, \, p^{(1)}_{\tau_1} = \left( q_{\tau_1}^{(1)} \right)^2,\, p^{(2)}_{\tau_2} = \left( q_{\tau_2}^{(2)} \right)^2,
\end{equation}
and with eq.~\eqref{eq:E65}
\begin{equation}
\label{eq:E71}
\begin{split}
\braket{s_k^{(1)}} &= q_{\tau_1}^{(1)} \left(\hat{S}_k \right)_{\tau_1 \rho_1} q_{\rho_1}^{(1)}\,, \quad 
\braket{s_k^{(1)} s_l^{(2)}} = \braket{s_k^{(1)}} \braket{s_l^{(2)}} \\
\braket{s_k^{(2)}} &= q_{\tau_2}^{(2)} \left(\hat{S}_k \right)_{\tau_2 \rho_2} q_{\rho_2}^{(2)}\,.
\end{split}
\end{equation}
The probability distribution \eqref{eq:E42E} for the classically entangled state cannot be obtained from a direct product normalized
classical wave function.

A general entangle classical wave function can be represented as a linear combination of direct product wave functions
\begin{equation}
\label{eq:E72}
q_\tau = \sum_a c_a q_{\tau_1}^{(a, 1)} q_{\tau_2}^{(a, 2)}\,.
\end{equation}
If we chose the direct product wave function orthogonal 
\begin{equation}
\label{eq:E73}
q_{\tau_1}^{(a, 1)} q_{\tau_1}^{(b, 1)} q_{\tau_2}^{(a, 2)} q_{\tau_2}^{(b, 2)} = \delta_{a b}\,,
\end{equation}
the normalization reads
\begin{equation}
\label{eq:E74}
\sum_a c_a^2 = 1\,.
\end{equation}
Every probability distribution can be represented in this way as $p_\tau = q_\tau^2$, including the one for the classically entangled
state \eqref{eq:E43E}. We observe complete analogy with entanglement in quantum mechanics.

\paragraph*{Three particle basis}

Following ref [55] we can represent the classical entangled state for $\Delta = 0$ by a direct product classical wave function. We
will generalize the setting and construct a classical probability distribution for which the correlation map to the two-qubit
quantum subsystem yields a pure entangled state of the form
\begin{equation}
\label{eq:E75}
\psi = \begin{pmatrix}
0 \\ \cos(\vartheta) \\ \sin(\vartheta) \\ 0
\end{pmatrix}\,.
\end{equation}
The maximally entangled quantum state \eqref{eq:E1} arises for $\vartheta = -\pi/4$. The non-vanishing quantum expectation values
or equivalent classical expectation values and correlations are given by
\begin{equation}
\label{eq:E76}
\begin{split}
\rho_{30} &= -\rho_{03} = \cos^2(\vartheta)-\sin^2(\vartheta)\,,\quad \rho_{33}=-1\,,\\
\rho_{11} &= \rho_{22} = 2\cos(\vartheta) \sin(\vartheta)\,.
\end{split}
\end{equation}

In the three-particle basis the classical spin operators are represented as
\begin{equation}
\label{eq:E77}
\begin{split}
\hat{S}_1^{(i)} &= t^{(i)} \otimes 1 \otimes 1\,, \quad \hat{S}_2^{(i)} = 1 \otimes t^{(i)} \otimes 1 \,, \\
\hat{S}_3^{(i)} &= 1 \otimes 1 \otimes t^{(i)} \,,
\end{split}
\end{equation}
with  diagonal $4 \times 4$ matrices.
\begin{equation}
\label{eq:E78}
t^{(1)} = \diag(1,1,-1,-1)\,, \quad t^{(2)} = \diag(1,-1,1,-1)\,.
\end{equation}
A direct product classical wave function takes the form
\begin{equation}
\label{eq:E79}
q_\tau = q_\alpha^{(1)}  q_\beta^{(2)} q_\gamma^{(3)}\,,
\end{equation}
with normalized four-component vectors $q_\alpha^{(k)} q_\alpha^{(k)} = 1$. One infers the expectation values
\begin{equation}
\label{eq:E80}
\rho_{k o} = \sum_\alpha t_\alpha^{(1)} \left( q_\alpha^{(k)} \right)^2\,, \quad 
\rho_{o k} = \sum_\alpha t_\alpha^{(2)} \left( q_\alpha^{(k)} \right)^2
\end{equation}
with $t_\alpha^{(i)}$ the appropriate eigenvalues of $t^{(i)}$. For the correlations one has
\begin{equation}
\label{eq:E81}
\begin{split}
\rho_{k k} &= \sum_\alpha t_\alpha^{(1)} t_\alpha^{(2)} \left( q_\alpha^{(k)} \right)^2\,, \\
\rho_{k l} &= \rho_{k o} \rho_{o l} \quad \text{for } k\neq l\,. 
\end{split}
\end{equation}
Taking 
\begin{equation}
q^{(1)} = q^{(2)} = \begin{pmatrix}
a \\ b \\ b \\ a 
\end{pmatrix}\,, \quad q^{(3)} = \begin{pmatrix}
0 \\ \cos(\vartheta) \\ \sin(\vartheta) \\ 0
\end{pmatrix}\,,
\end{equation}
with
\begin{equation}
\label{eq:E83}
a = \frac{1}{2}\left( \cos(\vartheta)+\sin(\vartheta)\right)\,, \quad 
b = \frac{1}{2}\left( \cos(\vartheta)-\sin(\vartheta)\right)\,,
\end{equation}
one realizes the entangled state according to eq.~\eqref{eq:E76}.

==> 2_5_6__Bells_inequalities.tex <==
\subsubsection{Bell's inequalities}

Bell's inequalities \cite{BELL}, or the more general form of the CHSH inequalities \cite{CHSH}, are identities for 
correlation functions in classical probabilistic systems. They become relevant for quantum subsystems if parts of the
probabilistic information contained in the quantum subsystem is given by classical correlation functions. This is the case
for the correlation map. In contrast, the average spin map employs no classical correlation functions. In this case the 
generalized Bell's inequalities only concern the environment. They are irrelevant for the quantum subsystem.

\paragraph*{Generalized Bell's inequalities and bit-quantum maps}

For the correlation map there is a set of quantum correlations, namely $\rho_{kl}$, that is given by classical correlation functions.
As for any classical correlation function they have to obey the CHSH inequality. Otherwise the correlation map cannot be a complete
bit-quantum map. If there would exist positive density matrices for which the quantum correlations $\rho_{kl}$ violate the
CHSH-inequality, this set of density matrices cannot be obtained from classical probability distributions. The only assumption for
the CHSH-inequality is the existence of some complete probability distribution for which simultaneous probabilities for the 
two factor in the correlations are available, and that the classical correlation is computed in the usual way using these simultaneous 
probabilities. We will show that the particular quantum correlations obey the CHSH-inequality. No obstruction to the completeness of the 
correlation map arises from this side. It is important that the particular set of quantum correlations $\rho_{kl}$ concern correlations
for commuting quantum operators. There exist other quantum correlations which violate the CHSH-inequality. They are not related to
classical correlation functions, such that no contradiction arises.

\paragraph*{CHSH-inequality}

For the relevant CHSH-inequality we employ two sets of classical Ising spins, namely $A, A'$ from the triplet of spins
$s_k^{(1)}$, and $B, B'$ from $s_k^{(2)}$,
\begin{equation}
\label{eq:E84}
\begin{split}
A &= \pm s_k^{(1)}\,, \quad A' = \pm s_l^{(1)}\,,\\
B &= \pm s_m^{(2)}\,, \quad B' = \pm s_m^{(2)}\,.
\end{split}
\end{equation}
We define the combination 
\begin{equation}
\label{eq:E85}
\begin{split}
C &= AB + AB' + A'B - A'B' \\
&= A \left(B+B'\right) + A' \left(B-B' \right)\,.
\end{split}
\end{equation}
Since $B$ and $B'$ are Ising spins with possible values $\pm 1$ one has either $B = B'$ or $B = -B'$. For $B' = B$ one has 
$C = 2AB$, such that $C$ can take the values $\pm 2$. For $B' = -B$ one finds $C = 2A'B$. Again $C$ can only take the values
$\pm 2$. For any probability distribution the inequality $-2 \leq \braket{c} \leq 2$, $\lvert\braket{c}\rvert \leq 2$, holds.
For a complete classical probability distribution the classical correlations $\braket{AB}$ etc. can be computed from the same
probability distribution as used for $\braket{c}$. One concludes the CHSH-inequality 
\begin{equation}
\label{eq:E86}
\lvert\braket{c}\rvert = \lvert \braket{AB} + \braket{AB'} + \braket{A'B}- \braket{A'B'}\rvert \leq 2\,.
\end{equation}
